Evaluation of Resource-Efficient Crater Detectors on Embedded Systems

Real-time analysis of Martian craters is crucial for mission-critical operations, including safe landings and geological exploration. This work leverages the latest breakthroughs for on-the-edge crater detection aboard spacecraft. We rigorously benchmark several YOLO networks using a Mars craters dataset, analyzing their performance on embedded systems with a focus on optimization for low-power devices. We optimize this process for a new wave of cost-effective, commercial-off-the-shelf-based smaller satellites. Implementations on diverse platforms, including Google Coral Edge TPU, AMD Versal SoC VCK190, Nvidia Jetson Nano and Jetson AGX Orin, undergo a detailed trade-off analysis. Our findings identify optimal network-device pairings, enhancing the feasibility of crater detection on resource-constrained hardware and setting a new precedent for efficient and resilient extraterrestrial imaging. Code at: https://github.com/billpsomas/mars_crater_detection.

==> tab/yolo_comp.tex <==
%------------------------------------------------------------------------------
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccccc} \toprule
\Th{Network}          & \Th{\#params}  & \Th{GFLOPS} &\Th{Init} & \Th{Accuracy} & \Th{\#params} \\ \midrule
\textsc{Base}         & GAP           & 12 & 12 & 73.3  & 22.1M \\ \midrule
\textsc{Base}         & \mr{6}{\cls}  & 12 & 0 & 72.7  & 22.1M \\
$\textsc{Base} + 1$   &               & 13 & 0 & 73.2  & 23.8M \\
$\textsc{Base} + 2$   &               & 14 & 0 & 73.7  & 25.6M \\
$\textsc{Base} + 3$   &               & 15 & 0 & 73.8  & 27.4M \\
$\textsc{Base} + 4$   &               & 16 & 0 & 73.9  & 29.2M \\
\rowcolor{LightCyan}
$\textsc{Base} + 5$   &               & 17 & 0 & \bf{74.6}  & 30.9M \\ \midrule
\rowcolor{LightCyan}
\textsc{Base}         & \mr{4}{\ours} & 12 & 12 & \bf{74.3}  & 22.3M\\
$\textsc{Base} - 1$   &               & 11 & 11 & 73.9  & 20.6M\\
$\textsc{Base} - 2$   &               & 10 & 10 & 73.6  & 18.7M\\
$\textsc{Base} - 3$   &               & 9 & 9 & 72.5  & 17.0M\\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\emph{Trade-off between performance and parameters}. Supervised pre-training of ViT-S on \imagenet for 100 epochs. \Th{Init}: Initial layer of pooling token. \textsc{Base}: original network. \textsc{Base}$+b$ (\textsc{Base}$-b$): $b$ blocks added to (removed from) the network.}
\label{tab:param}
\end{table}
%------------------------------------------------------------------------------

==> tex/related_old.tex <==
\vspace{-5pt}
\section{Related Work}
\label{sec:related}

% P1_pillar
% crater detection methods
% -manual
% -CDA's
% -DL technologies
\hspace{1.5em}\textbf{Crater Detection}
In the pursuit of efficient crater detection across planetary surfaces, methodologies have evolved from \emph{manual inspection} by experts to \emph{automated algorithms} and, more recently, \emph{deep learning}. Initially, planetary geologists manually inspected high-resolution images to identify and catalog craters\cite{standards_1979}. This method, though foundational, was limited by \emph{subjective interpretation} and lacked scalability for large-scale surveys.

%In the pursuit of efficient crater detection across planetary surfaces, various methodologies have been explored, ranging from \emph{manual inspection} by experts to \emph{automated algorithms} and, more recently, leveraging \emph{deep learning}. Traditionally, crater detection relied heavily on the expertise of planetary geologists who manually inspected high-resolution images to identify and catalog craters on planetary surfaces\cite{standards_1979}. This manual approach, while foundational, proved to be prone to \emph{subjective interpretation} among analysts and led to \emph{limitations} in scalability for large-scale surveys and comprehensive analysis of planetary surfaces.

In response to these challenges, automated \emph{crater detection algorithms} (CDA) have emerged. These algorithms employ various techniques such as the combinational Hough transform~\cite{CHT_Honda}, the continuously scalable template matching (CSTM)~\cite{template_matching}, shape recognition~\cite{shape_rec}, and processing highlight and shadow features using inverted images to eliminate non-crater features~\cite{bright_region}.

Detecting craters at large scales and across diverse diameters presents challenges, yet some studies have addressed these for global surveys~\cite{large_scale_DeLatte}. The advent of deep learning has further enhanced crater detection by allowing algorithms to develop their own features, resulting in improved efficiency and accuracy~\cite{large_scale_Silburt, DL, small_scale_DL, DL_review}. Recent deep learning methods utilize convolutional neural networks to automatically learn and extract features from training data, significantly advancing the field of crater detection.

% In response to these challenges, automated \emph{crater detection algorithms} (CDA) have emerged as a promising solution. Craters are detected by a two-step algorithm that first identifies round and symmetric topographic depressions  as potential crater candidates. Subsequently, a machine-learning technique is employed to confirm and select the actual craters. For instance, one approach based on Combinational Hough Transform is used to extract circular figures from binary images, using as parameters the center and radius of a circle\cite{CHT_Honda}. Another method known as The Continuously Scalable Template Matching (CSTM) algorithm as reported in \cite{template_matching} deploys templates to generate a model functioning within a user-defined range of continuous scales. A shape recognition algorithm that processes segmented images, optimized to be as noise-free as possible is utilized to efficiently identify the center location and dimension (radius) of each crater, ensuring precise results as detailed in \cite{shape_rec}. Another method, is processing highlight and shadow features simultaneously using an inverted image, eliminating all features that are not indicative of craters\cite{bright_region}. 

%In response to these challenges, automated \emph{crater detection algorithms} (CDA) have emerged as a promising solution. These algorithms employ various techniques such as the combinational Hough transform to extract circular figures from binary images~\cite{CHT_Honda}, the continuously scalable template matching (CSTM) algorithm for template-based crater detection~\cite{template_matching}, shape recognition algorithms for precise crater identification~\cite{shape_rec}, and methods that process highlight and shadow features using inverted images to eliminate non-crater features~\cite{bright_region}.

%\hspace{1.5em}\textbf{Crater Catalogues} 
%When considering Martian exploration, the first steps involved creating crater catalogues. Martian ground truth (GT) crater catalogues are derived from remote sensing data and annotated by experts, although in most scenarios the term GT refers to in-situ measurements.  Initial efforts to catalogue Martian craters \cite{Barlow1986, Rodionova2000, Boyce}, offered scientific insights while establishing the foundation for subsequent research, but later proved to be inconsistent due to duplicate entries and missing craters. The reason for this inconsistency is that they are not registered with up to date 1/1281 MOLA data, 1/2561 MDIM, 1/2561 THEMIS-DIR and 1/2561 MOC visual images. Two of the aforementioned approaches were merged into GT-57633 \cite{GT57633}, a catalogue with 57\,633 known Martian impact craters, particularly useful for CDA \cite{Bandeira2010, Harata, Stepinski} evaluation . 
% More recent researches show that larger craters rather than smaller ones are forming on Mars \cite{updated_catalog_Mars}.


\hspace{1.5em}\textbf{Benchmarking}
Accurately \emph{benchmarking} potential processing architectures is vital for ensuring these devices meet the \emph{computational demands} of modern edge applications, such as data processing, scientific measurements, autonomous navigation, and real-time decision-making. Simulating operational environments and stress-testing capabilities help identify potential failures and \emph{optimize} hardware and software configurations.  Given the constant advancements in developing more efficient devices, significant efforts review the state-of-the-art in embedded computing across various fields \cite{Naidoo2024}. Among edge applications, machine learning stands out due to AI's rapid growth and the need for low-latency, efficient data processing close to the source \cite{s23239495, woisetschläger2023fledge}.

Machine learning algorithms on spacecraft are particularly important for autonomous navigation and landing. The rise of commercially available embedded devices, which address increased processing needs while maintaining low power consumption, has garnered significant interest in the space community~\cite{glentar}. This is evident in application-oriented activities exploring these devices in specific mission scenarios, including earth observation and remote sensing~\cite{furano}, as also spacecraft pose estimation~\cite{aerospace7110159}.

%\subsection{Optical Navigation and Landing}
%application oriented
%optical navigation and landing 
%Unmanned Autonomous Vehicle (UAV) control


% For example, to use craters as landmarks to support motion estimation and precise landing, repeatability and viewpoint invariance are actually more important than whether the detected object is actually a crater or not.In assessing detection performance, it is frequently desirable to be able to analyze the results in various ways to discern the influence of various factors on the performance, e.g. by crater morphology, by terrain, by lighting, by size, by obliquity (viewing geometry).

% \cite{DIMES_landing}
% Hence, it is not surprising that there is still no CDA available that is as robust as the scientific community would like, and that several research groups are working in this still young field, trying to achieve this goal.

% \cite{space_yolo}
% Orbital images are particularly useful for capturing global, regional, and local contextual information, at a scale that cannot be achieved by a rover’s visual range
% For example, orbital images are used for landing site selection of ground missions, and to guide the path and daily operations of rovers such as Curiosity [e.g. Golombek et al., 2012; Stack et al., 2016]. Although the entire surface of Mars has been imaged by the Context Camera

% Ground images, on the other hand, offer a higher-resolution view of Martian terrains (down to the mm-scale) and provide “ground-truth” observations for orbital images. Ground-based images are needed to investigate the small-scale textural characteristics of outcrops, such as grain-size, lithology, internal sedimentary structures, or bedding styles, which are key for making depositional interpretations and paleoenvironmental reconstruction [e.g. Stack et al., 2016; Banham et al., 2018; Lewis and Turner, 2019; Stein et al., 2020]. However, in-situ observations of the Martian surface are limited to only eight surface mission locations (as of 2020).

% Such complementary datasets are also used for rover navigation, in particular to obtain precise rover localization [e.g. Parker et al., 2013; Weishu Gong, 2015] and to assist selection of rovers’ routes (e.g. minimizing traverses across wheel-damaging terrains [Arvidson et al., 2017])
